On Uniform Consistency of Spectral Embeddings

In this paper, we study the convergence of the spectral embeddings obtained from the leading eigenvectors of certain similarity matrices to their population counterparts. We opt to study this convergence in a uniform (instead of average) sense and highlight the benefits of this choice. Using the Newton-Kantorovich Theorem and other tools from functional analysis, we first establish a general perturbation result for orthonormal bases of invariant subspaces. We then apply this general result to normalized spectral clustering. By tapping into the rich literature of Sobolev spaces and exploiting some concentration results in Hilbert spaces, we are able to prove a finite sample error bound on the uniform consistency error of the spectral embeddings in normalized spectral clustering.

==> macros-thm.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}

==> yk-macros.tex <==
\def\Avar{\textrm{Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{\textrm{aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{\textrm{avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
%\def\bC{\mathbf{C}}
\def\bC{\boldsymbol{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\boldsymbol{F}}
\def\bff{\mathbf{f}}
\def\bG{\boldsymbol{G}}
\def\bH{\mathbf{H}}
\def\bI{\boldsymbol{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
%\def\bU{\mathbf{U}}
\def\bU{\boldsymbol{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\boldsymbol{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
%\def\bb{\mathbf{b}}
\def\bb{\boldsymbol{b}}
%\def\bc{\mathbf{c}}
\def\bc{\boldsymbol{c}}
\def\bbd{\mathbf{d}}
\def\bd{\textrm{bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\boldsymbol{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\boldsymbol{v}}
\def\bw{\boldsymbol{w}}
\def\bx{\boldsymbol{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{\textrm{Ber}}
\def\bin{\textrm{bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{\textrm{cat}}
%\def\Cov{\textrm{Cov}}
\def\Cov{\operatorname{Cov}}
\def\cov{\textrm{cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{\textrm{cl}}
\def\complex{{\bbC}}
\def\cone{\textrm{cone}}
\def\conv{\textrm{conv}}
\def\deq{\overset{d}{=}}
\def\det{\textrm{det}}
%\def\diag{\textrm{diag}}
\def\diag{\operatorname{diag}}
\def\diam{\textrm{diam}}
\def\dist{\textrm{dist}}
\def\dom{\textrm{dom}}
\def\doop{\textrm{do}}
\def\dto{\overset{d}{\to}}
\def\Ex{{\bE}}
\def\Exp{\textrm{Exp}}
\def\exp{\textrm{exp}}
\def\eg{{\it e.g.}}
\def\epi{\textrm{epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{\textrm{iid}}
\def\IID{\textrm{IID}}
\def\ind{\textrm{ind}}
%\def\intr{\textrm{int}}
\def\intr{\operatorname{int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{\textrm{KL}}
\def\ker{\textrm{ker}}
\def\lspan{\textrm{span}}
\def\maximize{\textrm{maximize}}
\def\med{\textrm{med}}
\def\minimize{\textrm{minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{\textrm{Poi}}
\def\Pr{{\bP}}
\def\peq{\overset{p}{=}}
\def\plim{\textrm{plim}}
\def\proj{\textrm{proj}}
\def\prox{\textrm{prox}}
\def\pto{\overset{p}{\to}}
\def\ran{\textrm{ran}}
\def\rank{\textrm{rank}}
\def\reals{{\bbR}}
\def\relint{\textrm{relint}}
\def\sign{\textrm{sign}}
\def\st{\textrm{st}}
\def\subjectto{\textrm{subject to}}
\def\supp{\textrm{supp}}
\def\symm{{\bS}}

\def\Tr{\textrm{Tr}}
\def\tr{\textrm{tr}}
\def\tube{\textrm{tube}}
\def\TV{\textrm{TV}}
\def\unif{\textrm{unif}}
%\def\Var{\textrm{Var}}
\def\Var{\operatorname{Var}}
\def\var{\textrm{var}}
\def\vct{\textrm{vec}}
\def\veps{\varepsilon}
\def\vol{\textrm{vol}}
%\def\zeros{\mathbf{0}}
\def\zeros{\boldsymbol{0}}

\def\Corr{\operatorname{Corr}}

\newcommand{\wF}{\widehat{F}}
\newcommand{\wG}{\widehat{G}}
\newcommand{\wL}{\widehat{L}}
\newcommand{\wbG}{\widehat{\bG}}

\newcommand{\indep}{\perp \!\!\! \perp}
\newcommand{\lin}{\operatorname{lin}}
\newcommand{\linfrac}{\operatorname{frac}}

\newcommand{\boldeta}{\boldsymbol{\eta}}
\newcommand{\tQ}{\widetilde{Q}}
\newcommand{\tpi}{\widetilde{\pi}}

\def\tk{\widetilde{k}}
